Supervisor Localization of Timed Discrete-Event Systems under Partial Observation and Communication Delay

We study supervisor localization for timed discrete-event systems under partial observation and communication delay in the Brandin-Wonham framework. First, we employ timed relative observability to synthesize a partial-observation monolithic supervisor; the control actions of this supervisor include not only disabling action of prohibitible events (as that of controllable events in the untimed case) but also "clock-preempting" action of forcible events. Accordingly we decompose the supervisor into a set of partial-observation local controllers one for each prohibitible event, as well as a set of partial-observation local preemptors one for each forcible event. We prove that these local controllers and preemptors collectively achieve the same controlled behavior as the partial-observation monolithic supervisor does. Moreover, we propose channel models for inter-agent event communication and impose bounded and unbounded delay as temporal specifications. In this formulation, there exist multiple distinct observable event sets; thus we employ timed relative coobservability to synthesize partial-observation decentralized supervisors, and then localize these supervisors into local controllers and preemptors. The above results are illustrated by a timed workcell example.

==> Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.25in,clip,keepaspectratio,scale = 0.8]{Figures/Zhang.eps}}]{Renyuan Zhang}
received the B. Eng. degree and the Ph. D degree in Electrical Engineering from
Xi'an Jiaotong University, Xi'an, China, in 2007 and 2013 respectively.
He is currently an Associate Professor at School of Automation, Northwestern Polytechnical University, Xi'an, China.
He was an international visiting student at the University of Toronto (2011-2012), and
a visiting researcher at Osaka City University (2015). His research interests
include distributed control of discrete-event systems and hybrid control of urban traffic systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.25in,clip,keepaspectratio,scale = 0.8]{Figures/Cai.eps}}]{Kai Cai}
received the B. Eng. degree in Electrical
Engineering from Zhejiang University, Hangzhou, China, in 2006; the M.A.Sc.
degree in Electrical and Computer Engineering from the University of
Toronto, Toronto, ON, Canada, in 2008; and the Ph.D. degree in Systems Science
from the Tokyo Institute of Technology, Tokyo, Japan, in 2011.
He is currently an Associate Professor at Osaka City University.
Previously, he was an Assistant Professor at the University of
Tokyo (2013-2014), and a postdoctoral Fellow at the University of
Toronto (2011-2013). 

Dr. Cai's research interests include distributed control
of discrete-event systems and cooperative control of networked multi-agent
systems. He is the co-author (with W.M. Wonham) of Supervisor Localization
(Springer 2015). He received the Best Paper Award of SICE in 2013,
the Best Student Paper Award of the IEEE Multi-Conference on Systems
and Control and the Young Author's Award of SICE in 2010.
\end{IEEEbiography}


==> SubSec_Relative_Coobs.tex <==

%\subsection{Formulation of Localization Problem}

{\color{red}
Now we have the new plant $\tilde{\bf G}$ to be controlled, new specification 
$\tilde{E}$ imposed on $\tilde{\bf G}$, and multiple subsets $\tilde\Sigma_{o, k}$ 
of observable events (rather than a single subset of observable events in Section 
III), as in (\ref{eq:new_observ_event}).
%So now we need the
%concept of `relative coobservability', which is closed under set union
%(thus there exists the supremal relative coobservable sublanguage of a given language
%and the supremal sublanguage can be effectively computed \cite{CaiEt:TAC2016}).
We first compute the supremal relative coobservable (and controllable and
$L_m(\tilde{\bf G})$-closed) sublanguage of $\tilde{E}\cap L_m(\tilde{\bf G})$,
and then apply the proposed partial-observation localization procedure
to construct partial-observation local preemptors and controllers.

%First, we briefly review the decentralized supervisory control proposed
%\cite{RudieWonham:1992} for the case that there exist multiple subsets of
%observable events.
%Let $P_k:\tilde\Sigma^* \rightarrow \tilde\Sigma_{o,k}^*$ be the
%natural projection as in (\ref{eq:natpro}) and $V_k: P_k(L_m(\tilde{\bf G})) \rightarrow
%Pwr(\tilde\Sigma)$ be the decentralized supervisor for each ${\bf G}_k$ $k \in \mathcal{N}$.
%We denote $V_{dec} = \wedge\{V_i|i \in \mathcal{K}\}$ the
%conjunction of the decentralized supervisors. Then the closed-loop system is
%$V_{dec}/\tilde{\bf G}$ \cite{RudieWonham:1992} with closed behavior $L(V_{dec}/\tilde{\bf G})$ and marked behavior
%$L_m(V_{dec}/\tilde{\bf G})$ ($:= L(V_{dec}/\tilde{\bf G}) \cap L_m(\tilde{\bf G})$).
%A supervisor $V_{dec} = \wedge\{V_k|k \in \mathcal{K}\}$ is {\it nonblocking}
%if $\overline{L_m(V_{dec}/\tilde{\bf G})} = L(V_{dec}/\tilde{\bf G})$, and {\it admissible}
%if for each $s \in L(V_{dec}/\tilde{\bf G})$, $k \in \mathcal{K}$,
%(i) $\tilde\Sigma_{uc,k} \subseteq V_k(P_k s)$ and
%(ii) $\big(Elig_{\tilde{\bf G}}(s) \cap V_k(P_k s) \cap \Sigma_{for,k} = \emptyset ~\&~
%tick \in Elig_{\tilde{\bf G}}(s)\big)~\Rightarrow tick \in V_k(P_k s)$,
%where $\tilde\Sigma_{uc,k} = \tilde\Sigma \setminus ({\tilde\Sigma_{hib,k}} \cup \{tick\})$.

%It is proved in \cite{RudieWonham:1992} that there exists a nonblocking and
%admissible supervisor $V_{dec} = \wedge\{V_k|k \in \mathcal{K}\}$ synthesizing
%$K\subseteq L_m(\tilde{\bf G})$, i.e. $L_m(V_{dec}/\tilde{\bf G}) = K$ if and only
%if $K$ is controllable, coobservable and $L_m(\tilde{\bf G})$-closed. When
%$K$ is not coobservable, there generally does not exist the supremal coobservable
%(controllable and $L_m(\tilde{\bf G})$-closed) sublanguage of $K$. Recently in \cite{CaiEt:TAC2016},
%a new concept of {\it relative coobservability} is proposed, which is stronger than coobservability but permits the
%existence of the supremal relatively coobservable sublanguage.

Let $C \subseteq L_m(\tilde{\bf G})$. A language $K \subseteq C$ is {\it relatively 
coobervable} (with respect to $C$, $\tilde{\bf G}$ and $P_k$, $k \in \mathcal{K}$, 
or simply $C$-coobservable, if for each $k \in \mathcal{K}$, $K$ is $C$-observable, 
i.e. for every pair of strings $s,s' \in \Sigma^*$ with $P_k s = P_k s'$ there holds
\begin{equation*}
(\forall \sigma \in \Sigma_{c,k}) s\sigma \in \overline{K}, s' \in C, s'\sigma \in 
L(\tilde{\bf G}) \Rightarrow s'\sigma \in \overline{K}.
\end{equation*}
where $\Sigma_{c,k} = \Sigma_{hib,k} \dot\cup \{tick\}$. For $\tilde{E} \subseteq 
L_m(\tilde{\bf G})$ as defined in (\ref{eq:new_spec}), write $\mathcal{CCO}(\tilde{E})$ 
for the family of controllable, $C$-coobservable, and $L_m(\tilde{\bf G})$-closed 
sublanguages of $\tilde{E}$. Then $\mathcal{CCO}(\tilde{E})$ is nonempty (the empty 
language $\epsilon$ belongs) and is closed under set union; $\mathcal{CCO}(\tilde{E})$ 
has a unique supremal element $\sup \mathcal{CCO}(\tilde{E})$ given by
\[\sup\mathcal{CCO}(\tilde{E}) = \bigcup\{K|K\in\mathcal{CCO}(\tilde{E})\}\]
which may be effectively computed \cite{CaiEt:TAC2015,CaiEt:TAC2016}.}
%Since relative coobservability is stronger than coobservability,
%$\sup \mathcal{CCO}(\tilde{E})$ is coobservable (controllable and $L_m(\tilde{\bf G})$-closed), and since relative
%coobservability is weaker than conormality, $\sup \mathcal{CCO}(\tilde{E})$ is generally
%larger than its conormality counterpart.


%% the end%%


==> SubSec_Supervisory_Control.tex <==

%\subsection{Supervisory Control under Partial Observation}

Supervisory control of TDES under partial-event observation was studied in \cite{LinWonham:1995}.
%where the concepts of timed observability and normality were introduced.
%We introduce timed relative observability \cite{CaiZhaWon:TAC2015}, which is stronger than timed observability,
%weaker than normality, and closed under set union.
Let $\Sigma_o \subseteq \Sigma$ be a subset of {\it observable} events, and
$P: \Sigma^* \rightarrow \Sigma_o^*$ the natural projection as in
(\ref{eq:natpro}). A {\it supervisor} $V$ under partial observation is any map
$V:PL_m({\bf G})\rightarrow Pwr(\Sigma)$. Then, the closed-loop system is
$V/{\bf G}$ \cite{Wonham:Book2015} with closed behavior $L(V/{\bf G})$ and marked 
behavior $L_m(V/{\bf G})$ ($:=L(V/{\bf G})\cap L_m({\bf G})$).
%
%
%Denoted by $V/{\bf G}$ the closed-loop
%system where ${\bf G}$ is under the supervision of $V$; the the closed language
%$L(V/{\bf G}) \subseteq L({\bf G})$ is defined inductively according to
%\begin{align*}
%&(i) ~\epsilon \in L(V/{\bf G}) \subseteq L({\bf G}); \\
%&(ii) ~s \in L(V/{\bf G}), \sigma \in V(Ps), s\sigma \in L({\bf G}) \Rightarrow
%       s\sigma \in L(V/{\bf G});\\
%&(iii) ~\text{No other strings belong to}~ L(V/{\bf G}).
%\end{align*}
%The marked language $L_m(V/{\bf G})$ of $V/{\bf G}$ is defined by
%\[L_m(V/{\bf G}) := L(V/{\bf G}) \cap L_m({\bf G}).\]
A supervisor $V$ is {\it nonblocking} if $\overline{L_m(V/{\bf G})} = L(V/{\bf G})$,
and {\it admissible} if for each $s \in L(V/{\bf G})$, (i) $\Sigma_{uc} \subseteq V(Ps)$;
(ii) $\big(Elig_{\bf G}(s) \cap V(Ps) \cap \Sigma_{for} = \emptyset ~\&~ tick \in
      Elig_{\bf G}(s)\big) \Rightarrow tick \in V(Ps)$,
%\begin{align*}
%&(i) ~\Sigma_{uc} \subseteq V(Ps); \\
%&(ii) \big(Elig_{\bf G}(s) \cap V(Ps) \cap \Sigma_{for} = \emptyset ~\&~ tick \in
%      Elig_{\bf G}(s)\big) \\
%&      ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\Rightarrow tick \in V(Ps),
%\end{align*}
where $Elig_{\bf G}(s):=\{\sigma \in \Sigma|s\sigma \in L({\bf G})\}$
is the subset of events `eligible' to occur (i.e. defined) at the
state $q = \delta(q_0, s)$.

It has been proved \cite{LinWonham:1995,Wonham:Book2015} that a nonblocking,
admissible supervisory control $V$ exists which synthesizes a (nonempty)
sublanguage $K\subseteq L_m({\bf G})$ such that $L_m(V/{\bf G}) = K$ if and
only if $K$ is observable, controllable and $L_m({\bf G})$-closed. While
controllability and $L_m({\bf G})$-closedness are properties closed under
set union, observability is not; consequently when $K$ is not observable,
there generally does not exist the supremal observable (controllable and
$L_m({\bf G})$-closed) sublanguage of $K$. Recently in \cite{CaiEt:TAC2016},
a new concept of {\it relative observability} is proposed, which is stronger
than observability, but permits the existence of the supremal relatively
observable sublanguage.

Now that $L_m({\bf G})$-closedness has been defined in (\ref{eq:Closedness}),
we introduce the definitions of controllability and relative observability as
follows. First, a sublanguage $K \subseteq L_m({\bf G})$ is {\it controllable}
\cite{BrandinWonham:94,Wonham:Book2015} if, for
all $s \in \overline{K}$,
\begin{eqnarray} \label{eq:control}
Elig_K(s)\supseteq
\left\{
   \begin{array}{lcl}
      Elig_{\bf G}(s)\cap(\Sigma_{uc} \dot{\cup}\{tick\}) \\
      ~~~~~~~~~~~~~~~~~\text{if} ~~Elig_K(s)\cap \Sigma_{for} = \emptyset,\\
      %~\\
      Elig_{\bf G}(s)\cap\Sigma_{uc}               \\
      ~~~~~~~~~~~~~~~~~\text{if} ~~Elig_K(s)\cap \Sigma_{for} \neq \emptyset,
   \end{array}
\right.
\end{eqnarray}
where $Elig_K(s):= \{\sigma \in \Sigma|s\sigma \in \overline{K}\}$
is the subset of eligible events after string $s$.
%Thus $F$ controllable means that an event $\sigma$ is eligible to
%occur in $F$ if (i) $\sigma$ is currently eligible in $\bf G$, and
%(ii) either $\sigma$ is uncontrollable or $\sigma = tick$ when there
%is no forcible event currently eligible in $F$.
Next, let $C \subseteq L_m({\bf G})$. A language $K \subseteq C$ is {\it relatively
observable} with respect to $C$ (or $C$-observable), if for every pair of strings
$s, s' \in \Sigma^*$ with $Ps = Ps'$ there holds
\begin{equation} \label{eq:def_relobs}
(\forall \sigma \in \Sigma_c) s\sigma \in \overline{K}, s' \in \overline{C},
s'\sigma \in L({\bf G}) \Rightarrow s'\sigma \in \overline{K}
\end{equation}
where $\Sigma_c = \Sigma_{hib} \dot\cup \{tick\}$. In the definition, the event
$tick$ is allowed to be unobservable, i.e. $P(tick) = \epsilon$.\footnote{
Note, however, that owing to the role of $tick$ in the TDES $\bf G$, $tick$ being
unobservable may render the observability condition difficult to be satisfied for
$K \subseteq L_m({\bf G})$.}

%A language $K' \subseteq K $ is {\it timed relatively observable}
%with resect to $\overline{K}$ (or {\it timed $\overline{K}$-observable}), if for every pair of strings $s,s'\in \Sigma^*$
%that are lookalike under $P$, i.e. $P(s)=P(s')$, the following
%two conditions hold \cite{CaiZhangWonham:2014b}:
%\begin{align}
%(i)~~&(\forall \sigma \in \Sigma) s\sigma \in \overline{K'}, s' \in \overline{K},s'\sigma\in L({\bf G})
%\Rightarrow s'\sigma \in \overline{K'} \label{eq:sub1:Treloberv} \\
%(ii)~~& s \in K', s' \in \overline{K} \cap \in L_m({\bf G})
%\Rightarrow s' \in K' \label{eq:sub2:Treloberv}
%\end{align}
For $E \subseteq L_m({\bf G})$, write $\mathcal{CO}(E)$ for the family
of controllable, $C$-observable, and $L_m({\bf G})$-closed sublanguages of $E$.
Then $\mathcal{CO}(E)$
is nonempty (the empty language $\epsilon$) and is closed under set union;
$\mathcal{CO}(K)$ has a unique supremal element $\sup \mathcal{CO}(E)$
given by
\[\sup\mathcal{CO}(E) = \bigcup\{K|K\in\mathcal{CO}(E)\}\]
which may be effectively computed \cite{CaiEt:TAC2015,CaiEt:TAC2016}.
Note that since relative observability is stronger than observability,
$\sup \mathcal{CO}(E)$ is observable (controllable and $L_m({\bf G})$-closed),
and since relative observability is weaker than normality, $\sup \mathcal{CO}(E)$
is generally larger than normality counterpart.

%% the end

